Physically Recurrent Neural Networks for Computational Homogenization of Composite Materials with Microscale Debonding

The growing use of composite materials in engineering applications has accelerated the demand for computational methods to accurately predict their complex behavior. Multiscale modeling based on computational homogenization is a potentially powerful approach for this purpose, but its widespread adoption is prevented by its excessive computational costs. A popular approach to address this computational bottleneck is using surrogate models, which have been used to successfully predict a wide range of constitutive behaviors. However, applications involving microscale damage and fracture remain largely unexplored. This work aims to extend a recent surrogate modeling approach, the Physically Recurrent Neural Network (PRNN), to include the effect of debonding at the fiber-matrix interface while capturing path-dependent behavior. The core idea of the PRNN is to implement the exact material models from the micromodel into one of the layers of the network. In this work, additional material points with a cohesive zone model are integrated within the network, along with the bulk points associated to the fibers and/or matrix. The limitations of the existing architecture are discussed and taken into account for the development of novel architectures that better represent the stress homogenization procedure. In the proposed layout, the history variables of cohesive points act as extra latent features that help determine the local strains of bulk points. Different architectures are evaluated starting with small training datasets. To maximize the predictive accuracy and extrapolation capabilities of the network, various configurations of bulk and cohesive points are explored, along with different training dataset types and sizes.

==> ann6.tex <==
\subsection{Network layout}
explain input damage to bulk (tractions would be fluctuating too much - doesnt make sense)

Damage is the internal variable stored in the cohesive points, which is either increasing or remains the same in case of unloading. This damage value modifies the local strain value that the bulk points receive, resulting in a modified value of local stresses for the same level of macroscopic strain. This gives rise to a modified tangent stiffness matrix that could capture the decrease in stiffness during unloading. The layout of the architecture can be seen in Figure \ref{fig:dam}, where in this case all bulk points receive the input damage from all the cohesive points when enlarging the network. This method also ensures that only the bulk points contribute directly to the stress homogenization procedure, unlike in the architecture from Section \ref{bch} with the cohesive points connected to the output directly by the decoder layer. To represent the non-linear relation between global strains and local displacement jumps, a custom activation function is applied at the cohesive point. The cohesive points are densely connected with the input layer through a linear relation and the resulting values of that are activated with a leaky ReLU function to obtain the final local displacement jumps. In that activation function, a bias term is considered. The idea of using the bias is to replicate the delayed displacement jump compared to the applied strain since the term allows for a shift of the function.

\begin{figure}[!h]
\centering
\includegraphics[scale=0.8]{elsarticle/Pictures/ann6s.pdf}
\caption{\centering Layout of a modified architecture with damage as input to bulk point}
\label{fig:dam}
\end{figure}

the displacement jumps that are passed to the cohesive points will be calculated by the following equation:

\begin{equation}
\llbracket \mathbf{u} \rrbracket = \phi^{(i)}(\mathbf{w_1} * \pmb{\epsilon}^{\omega} + \mathbf{b_1})
\end{equation}
with 
\begin{equation}
\phi^{(n)}(x, w, b) =
\begin{cases}
w \cdot (x-b) & \text{if } x \geq b \\
0.01 \cdot w \cdot (x-b) & \text{if } x < b
\end{cases}
\label{eq:leakymod}
\end{equation}
applied piece-wise on the normal component, and 
\begin{equation}
\phi^{(s)}(x, w, b) =
\begin{cases}
w \cdot (x - b + 0.01 \cdot b) & \text{if } x \geq b \\
w \cdot (x + b - 0.01 \cdot b) & \text{if } x \leq -b \\
0.01 \cdot w \cdot x & \text{otherwise}
\end{cases}
\label{eq:leaky_modsh}
\end{equation}
applied piece-wise on the shear component of the displacement jump. For physical interpretation of the activation function, the weight and bias values corresponding to the activation function at the cohesive points were forced to obtain positive values by applying a SoftPlus activation on the parameters. This, in theory, allows for a delay in damage initiation which corresponds to a positive bias value, and an increase of local displacement jump for increasing macroscale strain values.

\subsection{Predicting micro-scale damage}



==> prnn1.tex <==
\subsection{Network layout}
This section investigates whether the PRNN with the CZM in the existing material layer is able to capture micro-scale damage. This design choice preserves the same network architecture as previously discussed in Section \ref{prnn0}, and is the most straightforward extension of the network. Therefore, the PRNN proposed in this chapter consists of one input layer that receives macroscopic strains, one material layer with the nonlinear models, and one output layer yielding the macro-scale stress predictions (Figure \ref{fig:prnn1}). The nonlinear material models in the RVE are incorporated in the material layer by nesting them in bulk and cohesive fictitious integration points. Recall that 3 neurons represent one bulk integration point. \textcolor{red}{mention in intro that bulk is strain to stress} The cohesive integration points consist of 2 neurons, which are associated with a cohesive zone model to convert the local displacement jumps with normal and shear components to local tractions. Similar to the bulk points, the cohesive points also store internal variables to account for path-dependency. Along with the local strains and displacement jumps (depending on the type of material point), internal variables also serve as an input to the fictitious integration points. These material points are illustrated in Figure \ref{fig:ficmatpt}.

\subsection{Model selection}

To assess the network's performance in several loading scenarios, model selection was performed. The validation errors of the PRNNs were evaluated across different training sizes, comprising 32, 64, 96, 128, 160, and 192 non-monotonic and non-proportional curves. For each training set, different combinations of bulk and cohesive points were considered. The ratio of bulk to cohesive points was kept constant and equal to 4, mirroring the ratio of matrix to cohesive elements in the RVE. The size of the material layer ranged from a minimum configuration of four bulk and one cohesive points to 100 bulk and 25 cohesive points.

Figure \ref{fig:gpvalitr} displays the lowest validation MSE across the various training data sizes for the different material layer configurations. A training data size of 96 was selected, as the average value of the lowest MSE for different material layer sizes does not decrease significantly when further increasing the training size. Then, based on the MSE obtained on the validation set, a network with a combination of 4 bulk and 1 cohesive points was selected with a lowest MSE of 12.45 MPa. 

\begin{figure}[!h]
\centering
\includegraphics[scale=0.8]{Pictures/prnn1/trsize.png}
\caption{\centering Lowest validation MSE for different material layer sizes across various training data sizes}
\label{fig:gpvalitr}
\end{figure}

\subsection{Predicting micro-scale damage}

\begin{figure}[!h]
  \centering
  \begin{subfigure}[b]{0.47\textwidth}
    \centering
    \includegraphics[width=\textwidth]{elsarticle/Pictures/ANNv_41_96gp_nm64_14_1.png}
    \caption{\centering Prediction of network on a curve with low error}
    \label{fig:23gp72good}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.47\textwidth}
    \centering
    \includegraphics[width=\textwidth]{elsarticle/Pictures/ANNv_41_96gp_nm64_50_1.png}
    \caption{\centering Prediction of network on a representative curve}
    \label{fig:23gp72avg}
  \end{subfigure}

  \caption{\centering Prediction of network with 4 bulk and 1 cohesive points trained on 96 GP curves on test curves with one cycle of unloading}
  \label{fig:23gp72}
\end{figure}

Figure \ref{fig:23gp72good} shows that the selected network is able to capture the unloading phenomena in some cases. The stiffness of the unloading of the shear component of the prediction of the network is captured accurately. The monotonic region of these curves is also captured quite accurately.

Even though the considered networks are able to perform well in some cases, their prediction lacks consistent accuracy. Figure \ref{fig:23gp72avg} shows the prediction of the PRNN with 2 bulk and 3 cohesive points on a representative curve of the test set with an average test MSE of 9.27 MPa. The network not only misses capturing the decrease of stiffness during unloading but also loses accuracy on the monotonic part.

There is a large kink along the initial monotonic part of the curves shown in Figure \ref{fig:23gp72avg}, which is highlighted by red circles. Recall that the approximation of the network on macro-scale stresses is a result of a linear combination of the local stresses and tractions derived from the material model nested in the material layer. Figure \ref{fig:23gp72avg2} shows the microscopic stresses and tractions in the material points in the PRNN with 2 bulk and 3 cohesive points. For example, cohesive points $m_4$ and $m_5$ undergo tension, which is equivalent to what happens at the interface points where the fiber and matrix are debonding, while cohesive point $m_3$ undergoes compression. To account for the loss in stiffness due to microscale damage, the weights associated with the cohesive points are increased in magnitude so that the unloading branch of these curves can decrease the stiffness that would result from the plasticity model. However, as the weights associated with the cohesive points are increased, the contribution of the initial high dummy stiffness defined in the cohesive law is also increasing. Consequently, a large initial stiffness is observed in the macro response for small timesteps, which then causes the kink to appear on the curve. In the $\text{FE}^2$ method, introduced in Section \ref{fenn}, the micro-scale tractions computed by interface elements interact with the bulk points in the equilibrium equations of the RVE.  However, these micro-scale tractions do not contribute to the homogenized macro-scale stresses in the RVE, only the micro-scale stresses from the bulk points. In the PRNN discussed thus far, all types of nonlinearities were incorporated in the same material layer with the micro-scale tractions connected to the output with a dense layer. This arrangement does not allow for direct interaction between the micro-scale tractions and the bulk points, and as supported earlier by the kink phenomenon, the dense connection to the output layer poses some challenges. The current network architecture does not adequately represent the link between the cohesive and bulk points, nor does it capture the homogenization procedure. This conclusion leads to another important realization: while incorporating all sources of nonlinearity of the micro-model is necessary, it is not sufficient.  The architecture of the PRNN also must be carefully adjusted to better represent the underlying physics of $\text{FE}^2$ modeling. This conclusion leads to raise the question of whether there is an architecture of the PRNN with the plasticity model and cohesive zone model that is able to capture microscale damage. The following chapter focuses on designing different architectures of the PRNN to better represent the computation in the full-order micro-model, and on studying whether the proposed architectures are able to accurately predict micro-scale damage.
